Basis Adaptive Sample Efficient Polynomial Chaos (BASE-PC)

For a large class of orthogonal basis functions, there has been a recent identification of expansion methods for computing accurate, stable approximations of a quantity of interest. This paper presents, within the context of uncertainty quantification, a practical implementation using basis adaptation, and coherence motivated sampling, which under assumptions has satisfying guarantees. This implementation is referred to as Basis Adaptive Sample Efficient Polynomial Chaos (BASE-PC). A key component of this is the use of anisotropic polynomial order which admits evolving global bases for approximation in an efficient manner, leading to consistently stable approximation for a practical class of smooth functionals. This fully adaptive, non-intrusive method, requires no a priori information of the solution, and has satisfying theoretical guarantees of recovery. A key contribution to stability is the use of a presented correction sampling for coherence-optimal sampling in order to improve stability and accuracy within the adaptive basis scheme. Theoretically, the method may dramatically reduce the impact of dimensionality in function approximation, and numerically the method is demonstrated to perform well on problems with dimension up to 1000.

==> content/motivation.tex <==
\section{\texorpdfstring{Implementation Detail}{Problem Set Up}}
\label{sec:motivation}
%
\subsection{\texorpdfstring{The BASE-PC Iteration}{The BASE-PC Iteration}}
\label{subsec:iteration}

The BASE-PC iteration requires an initial basis, and set of samples. For our cases here the initial basis is a small basis containing relatively few elements and often being of significantly lower dimension than the overall problem. The initial set of samples is initially small, drawn from the $\ell_2$ coherence-optimal distribution in the initial basis. The iteration has three steps. The first is to identify samples for the current basis, drawn from a distribution which based on the assumption that the previous samples were drawn for the previous basis, leads to an aggregate pool of samples that is as if drawn for the current basis, insuring stability as the basis adapts, and as the corresponding desired sampling distributions change. The second step of the iteration is to identify a cross-validated surrogate solution in this basis from the aggregate pool of samples. The final step is to update the basis used to identify the surrogate using this surrogate solution. This iteration may be repeated until computational resources are exhausted, or when the cross-validated surrogate solution is sufficiently accurate for its necessary uses. In a scenario where the generation of new realizations of the QoI requires large amounts of time and computational resources, thus outpacing the iterative update of BASE-PC, this iteration can proceed until no reduction in cross-validated errors is observed or until new samples are available.

With this approach, $|\mathcal{B}|$ typically grows as the number of samples increased, and is shaped by anisotropy in order along each dimension. This allows certain dimensions to have a more stiff response with respect to the input random variables, and still be captured, without having to use high orders of approximation in all dimensions. Further, this gives a method for empirically identifying an appropriate level of stiffness for each input random variable, giving potentially useful physical information regarding the relationship of the QoI as a function of the input random variables.

We first consider the expansion in (\ref{Eq:PCETrunc}). For nomenclature, we refer to a basis function such that $|\mathbb{E}(u(\bm{\Xi})\psi_k(\bm{\Xi}))|$ is large as a necessary basis function, while a basis function with a relatively negligible expected inner product is called an ancillary basis function. Recall that $\mathcal{B}$ denotes the set of basis functions, i.e. $\{\psi_k\}_{k\in\mathcal{P}}$ used for computation at any particular computation. It is prudent to insure that $|\mathcal{B}|$ is large enough to include many necessary basis functions. Similarly, we seek to limit the number of ancillary basis functions to a number which is tractably small so that coefficients are estimated accurately. The extent to which a basis function is necessary or ancillary depends on the current state of the approximation insofar as a more accurate approximation will require more basis functions, and previously ancillary basis functions will become necessary to further reduce the error in the surrogate approximation.

To ensure a quality surrogate approximation we provide a method for identifying and generating the samples necessary to compute the coefficient vector $\bm{c}$ that is tractable and leads to stability in computation of the coefficients independently of basis. Further, we provide a consistent method for altering $\mathcal{B}$, that contains a high number of necessary basis functions while containing few ancillary basis functions. We briefly summarize these points, introducing the key theoretical guarantees. Each of these three steps have several parameters, and in Section~\ref{sec:examples}, the robustness is investigated on example problems.
%
\subsubsection{\texorpdfstring{Identifying Samples}{Identifying Samples}}
\label{subsec:id_samples}
We consider here a sampling distribution that improves concentration of the singular values of $\bm{D}$ around $1$, as in~\cite{Hampton15}. Let $w(\bm{\xi})$ be the weight associated with a sample, discussed in Section~\ref{subsec:sample_id}. We choose a distribution, minimizing a coherence parameter depending only on the basis functions being used, as well as any additional functionals of the QoI that are considered. This guarantees a stability of our computations using the design matrix.

As $\mathcal{B}$ adapts, the sampling distribution must change as well, and so too does its singular values. This raises a question concerning the fate of random variables generated for a basis set that does not coincide with the current computation. In Section~\ref{susubbsec:sample_id} a sampling is described, which allows a full reuse of previous samples, and at each step generates new samples so that the aggregate samples provides a minimization of the coherence parameter defined for the basis functions used in that computation, in a manner that mimics an independent sample from the coherence-optimal distribution. In this way we maintain a theoretically guaranteed stability in the condition number of the design matrix, and thus solutions computed from it remain stable. Specifically, when a convergence criteria is satisfied by the coherence-optimal sampling distributions, the following corollary shows that stability may be theoretically guaranteed when $N$ is taken to be linear in $|\mathcal{B}|$ up to logarithmic factors.
%
\begin{cor}
\label{cor:Sample_bound}
Assume that the sampling distribution associated with $\mathcal{B}_k$ converges to a limit as $k\rightarrow\infty$, in a manner described in the proof of Theorem~\ref{thm:sample_efficacy}. Then, for $\bm{D}_{k,\mathcal{S}}$, any submatrix of $\bm{D}_k$ formed by taking $|\mathcal{S}|$ columns in a set $\mathcal{S}$, it follows that for $k$ larger than some $k_0$
%
\begin{align}
\label{eqn:thm_efficacy_2}
\mathbb{P}\Bigg(\|\bm{D}_{k,\mathcal{S}}^T\bm{D}_{k,\mathcal{S}}-\bm{I}\|_2\le t+o(1)\Bigg)\le |\mathcal{S}|\mbox{exp}\left(-\kappa tN|\mathcal{B}_k|^{-1}\right).
\end{align}
\end{cor}
%
For specific work relating probabilistic bounds of this type to recovery by $\ell_1$-minimization we point the interested reader to related bounds in~\cite{CandesPlan,Hampton14,Peng16}.

It remains to identify how many samples should be generated to have a stable solution of (\ref{eqn:ell1}). It is sufficient to have a number of samples which scales linearly with $|\mathcal{B}|$, up to logarithmic factors, in a context that includes the QoI being a sufficiently smooth function of the input random variables. There is a robustness with regards to failure, but it is not theoretically impossible for the approximation to fail. If such robustness is needed, sampling can be increased until $\|\bm{D}^T\bm{D} - \bm{I}\|_{\sigma}$ is brought within a desired threshold such as for $\epsilon = 0.5$ where theoretical guarantees are available~\cite{CDL13}, but this may require a high computational cost both in verifying the condition and generating the necessary number of samples. The use of experimental design may be done to further improve this conditioning by further refining the samples drawn, but this is not considered here.

For approximating many practical QoI the number of required basis functions $|\mathcal{B}|$ scales favorably in dimension, specifically, higher order terms are only required in a relatively small number of dimensions. This is especially fortuitous in the event of exceptionally high dimensional problems, where there is decay in the importance of dimensions, although the rate of this decay may not be known, and the decay may not be monotonic. One way to identify such functions is by the anticipated decay in higher order terms. When this decay is exponential with regard to the order of the basis element in a manner that is consistent with an exponential decay with respect to the dimension of those basis elements. The main measure of error in this work is the RRMSE as defined in (\ref{eqn:RRMSE_def}).

To demonstrate this, if the following bound can be guaranteed for the coefficients, then to reach a particular RRMSE, $|\mathcal{B}|$ scales nearly linearly with dimensionality, and so too does the necessary $N$. Additionally, define $\tilde{u}$ to be the approximation in $\mathcal{B}$, that minimizes RRMSE$(\hat{u})$. Related to this, define $\mathcal{F}(\mathcal{B})$ to be the space of possible approximations built from $\mathcal{B}$, and then
%
\begin{align}
\label{eqn:u_tilde_def}
\tilde{u}_{\mathcal{B}} := \mathop{\mbox{argmin}}\limits_{\hat{u}\in\mathcal{F}(\mathcal{B})}\mbox{RRMSE}(\hat{u}).
\end{align}
%
Using this definition, we can show the following lemma.
%
\begin{lem}
\label{lem:curse_dimensionality_assumption}
Let $\bm{i}$ be the $d\times 1$ vector that indexes the order of the basis function in each of $d$ dimensions, and let $c_{\bm{i}} = |\mathbb{E}(u(\bm{\Xi})\psi_{\bm{i}}(\bm{\Xi}))|$ denote the corresponding coefficient for the most accurate reconstruction of the surrogate, $\hat{u}$. If there exists an $\alpha >0$ such that
%
\begin{align}
\label{eqn:curse_assumption}
|c_{\bm{i}}|\le \exp\left(-\alpha\mathop{\sum}\limits_{k=1}^d k i_k\right),
\end{align}
%
then for a prescribed $\epsilon >0$, there exists an anisotropic order basis, $\mathcal{B}$ such that $|\mathcal{B}| \le C\epsilon^{-\kappa}$, where $C$ is a universal constant, and $\kappa\ge0$. With $\tilde{u}_{\mathcal{B}}$ as in (\ref{eqn:u_tilde_def}), it follows that
%
\begin{align*}
\mbox{RRMSE}(\tilde{u}_{\mathcal{B}}) \le \epsilon.
\end{align*}
%
\end{lem}
%
Specifically, Lemma~\ref{lem:curse_dimensionality_assumption} guarantees that for a fixed accuracy of reconstruction the size of the basis needed for accurate reconstruction scales nearly linearly in $d$. Combined with Corollary~\ref{cor:Sample_bound}, we arrive at the following Corollary.
%
\begin{cor}
\label{cor:curse_break}
Let the assumptions of Lemma~\ref{lem:curse_dimensionality_assumption} and Corollary~\ref{cor:Sample_bound} be satisfied. Then there exists a basis $|\mathcal{B}|$ and a sample size $N$ such that, if $\mathcal{B}$ is the active basis, and the total number of samples $N$ is sufficiently large, then
%
\begin{align*}
\mbox{RRMSE}(\hat{u}) \le \epsilon.
\end{align*}
%
A number of samples to guarantee this accuracy is of order $\epsilon^{-\kappa}$, up to logarithmic factors.
\end{cor}
%
It is important to note that the bounds in Lemma~\ref{lem:curse_dimensionality_assumption} and Corollary~\ref{cor:curse_break} are independent of $d$, depending only on $\epsilon$, and that these bounds hold even for infinite $d$, as long as (\ref{eqn:curse_assumption}) holds. Also, though we can guarantee the existence of a quality basis, and guarantee accuracy with a favorable number of samples when using that basis, we can not theoretically guarantee that this basis can be identified within any number of iterations. Specifically, there are no guarantees that the quality basis can simultaneously be identified using the samples to generate the accurate solution, while those samples and the associated solution themselves inform the basis. In other words, the parts of the iteration arising from the following sections do not yet connect with the sampling machinery to guarantee theoretical convergence, or convergence with the rate given by Corollary~\ref{cor:curse_break}. However in Section~\ref{sec:examples}, the iteration is numerically investigated on examples, showing favorable decay. It is expected that improvements to the procedure can further improve the rates, but theory incorporating the entire iteration remains undeveloped.

Further this bound in terms of $\epsilon$ can be seen to grow quite quickly as $\epsilon \rightarrow 0$, as the number of necessary basis functions increases dramatically to capture larger numbers of basis functions with smaller contributions. Also, this exponential decay in dimensionality is quite strict for a requirement, and may not hold for many practical purposes. However, the result does suggest that as long as there is a decay in the coefficients associated with higher dimensions that a significant reduction in the dependence of the number of samples on dimension may be expected.

\subsubsection{\texorpdfstring{Computing Cross-Validated Solution}{Computing Cross-Validated Solution}}
\label{subsec:cross_validation}
While solutions to our matrix problem are identified by (\ref{eqn:ell1}) using a modified version of SPGL1~\cite{spgl1:2007}, we require an identification of $\delta$, to produce a solution with as much accuracy and as little overfitting as possible. Unless otherwise stated we compute solutions using 24 independently generated folds of available samples, using the same folds for each $\delta$ at each iteration. For each fold and $\delta$, we use 80\% of the samples to compute the solution, and 20\% of the samples to estimate the RRMSE associated with that $\delta$ and its fold. Averaging the RRMSE over all folds gives the estimate for that $\delta$, and we select the $\delta$ that returns the lowest average RRMSE, using this $\delta$ to compute the updated solution from the full pool of samples. The set of potential $\delta$ is $0$ and then a set of $20$ tolerances that are evenly spaced in a logarithmic scale between a minimum tolerance of exp($-2)$ or $c$exp($\delta_0$), and a maximum tolerance of exp($(c+1)\delta_0$). Here $\delta_0$ is the maximum of the previous RRMSE or previously validated tolerance, and $c$ is chosen to be $1.5$ in the computed examples.
%
\subsubsection{\texorpdfstring{Altering the Basis Set}{Altering the Basis Set}}
\label{subsec:basis}
If we have a previously selected basis set $\mathcal{B}_0$, and a corresponding computed coefficient vector $\bm{c}_0$, then heuristically we reduce $\mathcal{B}_0$ to $\mathcal{B}_1$ by keeping those elements corresponding to large coordinates $|\mathcal{c}_0|$, and removing those elements corresponding to small coordinates in $|\mathcal{c}_0|$. This is closely related with the variance informed refinements in~\cite{Wan05}, where here we typically have higher orders in dimensions with more unexplained variance. Using a single loop over the defined basis, we define for each basis function $i=\{1,\cdots,|\mathcal{B}_1|\}$, $k_{j}$ for $j=\{1,\cdots,d\}$ corresponding to the order in each dimension. We then define $\bm{p}$ as in (\ref{eqn:general_order_def}) to be the coordinate wise maximum of $\bm{k}$, and define $\mathcal{B}_2$ as the anisotropic order basis defined by $\bm{p}$. The following lemma shows that under a certain convexity requirement for $\bm{c}$ with respect to $\mathcal{B}_1$, this is the definition or anisotropic order minimally contains all elements in $\mathcal{B}_0$, but in absence of this may remove a few necessary basis functions. By itself this is usually insufficient to preclude a quality approximation, but severe violations of this convexity may mean certain necessary basis functions are never reached by BASE-PC, and hence never have an opportunity for inclusion.  It should also be noted that exceptional decay rates may produce a need for a large number of samples for accurate basis identification due to $\ell_1$-minimizations selection of sparse solution vectors, reducing the inclusion of the necessary higher-order basis functions.
%
\begin{lem}
\label{lem:basis_convexity}
Let $\bm{i}$ denote the order for a basis function in dimension $1:d$, and let $c_{\bm{i}}$ denote the corresponding coefficient in the approximation at any given step. Define the weighted norm
%
\begin{align}
\label{eqn:norm_def}
\|\bm{i}\|_{\star} := \mathop{\sum}\limits_{k=1}^d \frac{i_k}{p_k}.
\end{align}
%
If the vector of $p_k$ in (\ref{eqn:norm_def}) is chosen to be $\bm{p}$ as defined above, then the proposed anisotropic order basis is defined by including all basis functions satisfying $\|\bm{i}\|_{\star}\le 1$. If for all $\bm{i}\in\mathcal{B}_0$,
%
\begin{align}
\label{eqn:bound}
\|\bm{i}\|_{\star} \le 1,
\end{align}
%
then $\bm{p}$ defines the anisotropic order basis of minimal size which contains all basis elements in $\mathcal{B}_0$. Specifically, $\mathcal{B}_2$ is the anisotropic order set of smallest size which contains $\mathcal{B}_0$.
\end{lem}
%
The contracted basis $\mathcal{B}_2$ is expanded to an anisotropic order basis $\bm{p}_2 := \lceil(1+\rho)\bm{p}_1\rceil$, where $\rho$ is a user defined expansion rate, and unless otherwise stated we take $\rho := 0.01$, which increases each order by $1$, and is appropriate for low order cases. For cases with very high order, many iterations would be needed to identify an appropriate order, and in this case $\rho$ should be increased. If there are unused higher dimensions, corresponding to $p_i=0$, then a predefined number of new dimensions are added to the approximation at each iteration, where this number here is $2$ or $20$ depending on the dimensionality of the problem. It is also possible to enforce lower and upper bounds on the order $\bm{p}_2$, which reduces the change in the basis which provides more stability. This approach is robust in that discarding a necessary basis function is not catastrophic, as there is a high probability of it being reintroduced when more data is available, or when the basis is readjusted even with the same data. 

Critically, the precise selection of basis functions included is determined only by problem prescribed data and realized data from evaluations of the QoI, allowing a ubiquity in potential applications. Further, as long as there is decay with regards to the relative importance of dimension in explaining the QoI, a valid assumption in many cases, then there is the potential for dramatic reduction in the number of basis functions used to construct the surrogate approximation. This framework produces a less-refined adaptivity to the basis than the methods of~\cite{Blatman11, Jakeman15}, which evaluate inclusion for individual basis functions. Heuristically, while a degree of basis efficiency is needed to capture desired basis functions, a benefit of compressed sensing is that a reasonable number of ancillary basis functions are acceptable, motivating the broad scope of the basis search seen here, and so the relaxation from individual basis functions to the $d$-parameters defining the anisotropic orders is often acceptable in terms of computational efficiency.

We modify this approach to further improve stability and accuracy in the computed solution by selecting from a number of potential bases the one that has the minimal error. Specifically, basis functions are removed from the truncated basis based on a sorting of $|\mathcal{c}_0|$ until changes would be seen in the expanded basis, and then a solution is computed in this new basis from the available samples, with a corresponding validated error. This may be implemented efficiently, given that it is possible to test effectively when a removed basis function changes $\bm{p}_1$, which in turn imparts a change to $\bm{p}_2$ that may be incorporated into the already computed basis by removing the required basis functions. The basis producing the minimum cross-validated error is kept, where we cease trying bases after a number of consecutively tested bases are above the minimal realized error. It is likely that the decay in validated error is not entirely monotonic, especially when considering the statistical nature of the cross-validated error estimate, so this makes the estimate more robust. This approach allows a broad search of potential bases, and reduces the need to tune parameters related to the basis adaptation. In addition, this iteration of expansion/contraction is attempted up to three times before new samples are added, where it is stopped early if the basis of one iteration matches that of a previous iteration.
